Anception: Application Virtualization For Android

The problem of malware has become significant on Android devices. Library operating systems and application virtualization are both possible solutions for confining malware. Unfortunately, such solutions do not exist for Android. Designing mechanisms for application virtualization is a significant chal- lenge for several reasons: (1) graphics performance is important due to popularity of games and (2) applications with the same UID can share state. This paper presents Anception, the first flexible application virtualization framework for Android. It is imple- mented as a modification to the Android kernel and supports application virtualization that addresses the above requirements. Anception is able to confine many types of malware while supporting unmodified Android applications. Our Anception- based system exhibits up to 3.9% overhead on various 2D/3D benchmarks, and 1.8% overhead on the SunSpider benchmark.

==> arch.tex <==

\subsection{Management of Apps and Containers}
All Android apps are started by a fork from the Zygote process. After the fork, Zygote specializes the child into an application by setting its
uid and other parameters. We added code to notify the Anception kernel module of this, and we replicate the same on the guest by spawning a proxy, and specializing it.
A userspace daemon executes on the host and is responsible for VM management functions like startup and shutdown. It communicates
with the host module through a miscellaneous device node. It is also responsible for binding an application to a container by setting its
\texttt{vmid} flag to a valid index in the redirection vector. 
The {\tt vmid} flag identifies the Container ID associated with the app.
A value of 0 for {\tt vmid} identifies the trusted host. Higher
values identify the application's container.  


This {\tt vmid} value is added as a one byte field in the process descriptor in
the host kernel so that a process's container can be identified by the
system.  This does limit Anception to at most 256 containers, 
but that is likely to be more than sufficient in practice.

When an app runs, the Anception kernel module obtains the
\texttt{task\_struct} of the process, and sets the virtualization byte
({\tt vmid}) to the appropriate index value. The vmid is inherited by
a process's children. Forking/cloning does not allow a process to
escape its container. Also, since this process descriptor is
maintained on the host side, compromise of a root service in the
container does not allow the app to change its {\tt vmid} and escape
the container.


\subsection{Container Implementation}
Containers run a special version of Android that contains the stock
Android system in a guest virtual machine.  It has all the core
userspace system services found in a regular Android system. The
window manager and input manager are nullified by making them talk to
dummy devices. Thus, the capability to render and process touch input
is nullified. We refer to this as {\em headless} Android. 
The point of running this in the guest VM is to provide an alternate,
mostly-identical system view to an untrusted process.

Note that apps are not installed inside container images. Thus,
all container images are essentially identical, except for state
of the apps that are bound to the containers. Furthermore, most
of the runtime state of apps resides outside the container, since
the memory pages of apps mostly reside in the host (except for 
much smaller state of the corresponding proxy that runs in the container).

The above design allows the run-time memory footprint of Anception
containers to be much smaller than solutions that do full
virtualization, including Cells~\cite{cells}, which is especially
designed to have small memory footprint.

\subsection{Proxies in an Anception Container}
An app's system call must be forwarded to its proxy (which runs in a guest
container). When a proxy is first started, it is 
granted the same uid (among other parameters like umask). When a redirected system call arrives at the proxy, we need
an efficient way of delegating its execution to the proxy. This means we have to transfer execution from kernel context to the proxy's process
context. One could have a message passing mechanism that notifies a userspace process upon receipt of a system call from the host, but this
would require four costly context switches to complete. 

%\hl{Please check this. The last few sentences in the para below are confusing}
Anception uses a more efficient technique that eliminates two of the
context switches. We force the proxy process to enter an
\textit{interruptible sleeping wait} in kernel space through an ioctl
on its container's kernel module. When a redirected system call comes
in, we post this call to the container's kernel, which in turn wakes up the 
target proxy. After execution of the system call is complete (without leaving 
the container kernel), the proxy goes back to sleep, in kernel space. 
This mechanism saves us two context switches over the
other option of having the proxy wait in userspace for a notification
from the container's kernel that a system call is to be executed. 



\subsection{Efficient System Call Interception}

To be able to redirect system calls, one must first intercept a system
call. We tried out several system call interception mechanisms --  in particular
{\tt ptrace}, {\tt kprobes}, {\tt frace}, {\tt dtrace}, and {\tt utrace} --
 but found them to be too slow or limiting. For example, Anception's first prototype was built using \texttt{ptrace} and User-Mode Linux \cite{uml}.
In this experiment, we bound untrusted processes by ptrace-ing them. However, microbenchmark tests indicated overheads upwards of
60x (primarily due to a high number of context switches). 
In Android, all applications derive from Zygote. During a ptrace session, reparenting occurs, and this may cause unintended side-effects. Other mechanisms,
primarily debugging or tracing mechanisms, were also not efficient
enough for our purposes.

\begin{comment}
\begin{itemize}
\item \texttt{kprobes} are a debugging mechanism that allows
setting of hooks at any code address of a running kernel. We could set up a break point at the system call interrupt handler,
and then have our logic execute. The problem with this is that there is some context saving \footnote{in addition to the state saving done by the system gate} 
to be done to correctly execute a kprobe. The bigger problem is that setting a kprobe affects the whole system. Any process hitting
the kprobe will jump to the handler, and not just those bound to an Anception container.

\item \texttt{ftrace, dtrace, utrace} are kernel level mechanisms to trace kernel functions including system calls. These are intended to
aid in debugging and are not efficient enough to be used on critical paths like the system call entry handler.

\end{itemize}
\end{comment}

We decided to design our own system call interception mechanism that was 
suited for transferring the call to a proxy process in a different container
efficiently.
The system call interception mechanism incurs an overhead of just a few
instructions on the host system.

The basic insight was that we could create a different system call
table per container and then provide an efficient way of redirecting a
system call to the appropriate table, based on the app's container ID
(which is available in the {\tt vmid} value in the process
descriptor as described in part B). 

\begin{comment}
These alternate tables serve as stubs, and can be
filled in by writing virtualization dependent code. This is termed as
the {\em VM-bridge} (see Figure \ref{arch1}) and it depends on the
type of virtualization technology we use. VM-bridge code is also part of
the Anception kernel module.  Anception uses lguest \cite{lguest},
which is a very small research hypervisor for the x86 platform, that
requires no specific hardware support beyond protection rings.
\end{comment}

\begin{comment}
To achieve high efficiency in intercepting and redirecting, Anception
virtualizes the system call interface for processes by adding a
\textit{virtualization byte} to the process descriptor.  As we see in
Figure \ref{syscallres}, when a host Linux process (untrusted app)
executes a system call instruction (\texttt{int 80, sysenter}),
control is transferred to the system interrupt handler. 

At this point, after sanity checks, an index calculation is performed
that results in calling of the actual system function. Anception
modifies this path by adding an extra check ($vmid > 0$, see Figure
\ref{syscallres}). 

 If its value is greater
than 0, it represents an index into the \textit{Redirection Vector}
(RV), which is an array of pointers. The RV's pointers point to
alternate system call tables that redirect the call to the app's proxy
in the appropriate container.
\end{comment}

\begin{comment}
When an app runs, the Anception kernel module obtains the
\texttt{task\_struct} of the process, and sets the virtualization byte
({\tt vmid}) to the appropriate index value
 into the redirection
vector. Therefore, setting the virtualization byte in the process
descriptor allows us to virtualize the entire system call interface
for a process by setting just one byte.
\end{comment}


Figure \ref{arch1detail} shows the details of a system call.  When an
application process makes a system call (step 1), control is
transferred to the system call interrupt handler (step 2). At that
stage, we analyze a field in the process descriptor, named
\texttt{vmid}, that allows us to identify the container that is bound
to the process. A value of 0 indicates that the process runs directly
on the trusted host and no redirection should occur. If {\tt vmid} is
greater than 0, its value specifies an index into a redirection
array. The redirection array is a set of base addresses for various
system call tables corresponding to the various containers. The
implementations of system calls will serialize call arguments (step 3)
and transfer them to the guest kernel via the \texttt{virtio}
transport (step 4).  Once the call has been executed by the host
process's proxy, the results are returned either via \texttt{virtio}
or via a hypercall (step 5). Finally, the results are returned to the
original process that initiated the call.

\begin{comment}
This mechanism is highly efficient and
microbenchmark tests indicate that the extra x86 assembly we have
written for this adds negligible overhead.
\end{comment}


\begin{comment}
host side module
-- syscall interception, virtualization byte
-- tried UML with ptrace
-- kprobes - but affects whole system, ours only marked processes
-- no race because VM started and syscall table set up before process starts executing
-- inheritance of virt byte

-- transfer mechanism virtio natural choice used by many, hypercall

guest side venus module, viced, proxy, configuration identical
venus mode - give a kthread temporary process context - not work.
post messages thru IPC - too much overhead, sleeping wait - works best.

manager process, app launch, Zygote forking

binder ioctl identification
\end{comment}

\begin{figure}[ht!]
\center
\includegraphics[width=3.3in,height=3.6in,keepaspectratio]{images/arch_detail1.pdf}
\caption{Anception Architectural Detail}
\label{arch1detail}
\end{figure}


System call interposition has been the topic of much research in the
past, several problems have been identified
\cite{Garfinkel03trapsand}, and solutions have been developed
\cite{Garfinkel03ostia:a, Venkatakrishnan03isolatedprogram}. Our
system call interposition method follows several best practices
outlined in previous research \cite{Garfinkel03ostia:a,
  Venkatakrishnan03isolatedprogram, Laadan:2010:OSV:1815695.1815717},
while avoiding the problems encountered while building systems such as
in \cite{janus,
  Jain99user-levelinfrastructure}.  Some representative problems
include time-of-check-time-of-use (TOCTOU) attacks, and symlink races.
The choice of which syscalls to intercept has been influenced in part
by the REMUS system~\cite{Bernaschi:2002:RSO:504909.504911}.

\begin{comment}
The above problems generally occur when interposition makes an access control decision based
on system call arguments but malware has some control over the target of the arguments. For
example, a system call may be provided a symlink as a parameter that initially points to
a permitted file. The system permits that action. Malware then switches the target of the file
to a sensitive file. The system allows the file to be opened, even though that should have been
denied. We do not believe our design for system calls to be vulnerable to TOCTOU attacks
because its job is to simply copy the arguments of the system call verbatim,
and send them to the guest. Anception does not perform access control decisions
on the arguments. In the cases where we make a decision about whether
redirection is performed or not, we always expand any symlinks and
copy their target filename immediately to kernel space upon a system call.
\end{comment}

Our streamlined implementation of system call interception adds a few
assembly lines to the system call interrupt handler. In practice, this
is efficient. Furthermore, the amount of architectural state we save
to intercept and redirect is negligible. For details, see Table
\ref{archsave}. The minimal runtime overhead of the system call interception is reported
in Section \ref{perf}.

\begin{table}[ht!]
\center
\begin{tabular}{| l | l | l |}

   	\hline
  	entry method		&			save																			&	restore \\ \hline	
  	int 80				  &  movl \%eax, \%ebx															& movl \%ebx, \%eax \\ \hline
  	
  	\multirow{4}{*}{sysenter} & pushl \%esi				 					& popl \%esi \\ 
  														& pushl \%ebx									& popl \%ebx \\
  														& pushl \%ecx									& popl \%ecx \\
 															& movl \%eax, \%ebx 					& movl \%ebx, \%eax \\ \hline
  	 																																		
  	
\end{tabular}
\caption{Architectural State Saves}
\label{archsave}
\end{table}

\begin{comment}
The Anception modified handler extracts a identifier byte from the process descriptor. We modified the process descriptor
\texttt{task\_struct} to include this new field. This field is inherited by all spawned children.
During host module initialization, various alternate stub 
system call tables are set up. 
\end{comment}

\vspace{-0.2in}


\begin{comment}
The challenging aspect of virtualizing the system call interface on a
per process level is doing it efficiently. Unlike resources such as
process memory that are managed on a per-process level, the system
call table has always been a whole system resource. All processes see
the same system call table. Therefore, making changes to it will cause
performance degradation for all processes that invoke system calls.
\end{comment}

\begin{comment}
\begin{figure}[ht!]
\center
\includegraphics[width=2.8in,height=1.5in,keepaspectratio]{images/syscall_res1.pdf}
\caption{System Call Resolution}
\label{syscallres}
\end{figure}
\end{comment}

%\input{redirection}


%With diagram describe arch. Interleave discussions
%of assume this...then this happens situations thus showing
%how useful this system is and how it saves the world. Helps
%to show why certain architectual features exist.
%Stress disconnection from virtualization technology.

\begin{comment}
Therefore,
the question we try to answer with Anception's architecture is, ``How do you adapt an existing
technology to a smartphone environment while at the same time tune it to the intricacies of these
devices?". 
\end{comment}


% We use type II virtualization wherein the guest VM appears as a
%set of processes on the host OS. Thus scheduling and resource usage
% are controlled by the host OS.

%The job of the VM-bridge code is to serialize system call arguments, much like the trusted thread in
%the seccomp sandbox \cite{seccomp}, and transport them to the guest virtual machine, where they are executed,
%and then bring back the results. Anception uses virtio \cite{virtio}, which is a standard method of
%communicating with guest virtual machines.

%The guest virtual machine (see Figure \ref{arch1}, right hand side) is a copy of the host system but without the ability to write to the framebuffer. It is
%a headless instance with an identical kernel and userspace stack. It doesn't have the ability to receive
%incoming touch (or gesture) input as well. The reason for this is twofold. 
%First it achieves our first design goal of a unified user experience, where user interaction model is unchanged. 
%And second, a headless guest VM has a reduced memory footprint on the host.

\begin{comment}
The first is that we want to 
unify the user experience, and in doing so, keep the interaction model with users the same. The common
user is accustomed to seeing a single application, clicking on it, and having it launch. This is a standard UI
paradigm. We do not want to change this experience in a fundamental way, like other solutions \cite{cells}. 
The second reason for the guest VM being headless is that we reduce its memory footprint.
\end{comment}


%The window managers consume XX\% of the total memory of an Android system. By choosing to not have a window
%manager, we save this memory. 


==> designgoals.tex <==
\section{Design Goals}
\label{sec:designgoals}
%re-use existing security mechanisms of android andlinux kernel
%provide easier UI management of multiple "worlds" by intelligent
%redirection. App compatibility.
Our design goals are as follows:

\begin{comment}
\begin{itemize}
\item Protect the host OS and its trusted applications from untrusted apps.
\item Not require changes in the way users interact with apps in
  standard mobile OS (in our case, Android).  Requiring significant
  changes from users due to security can be a disincentive for
  adoption of security solutions.  For example, if users were required
  to manually switch among different sandboxes to switch among apps,
  the extra cognitive burden may cause users to simply keep all apps
  in a single sandbox, defeating the security goals.
\item Re-use the existing security principles of the Linux kernel and Android stack.
\item Keep the architecture simple and implementation small with minimally invasive changes to the host OS.
\item Provide high perforamnce, especially for interactive apps.
\end{itemize}
\end{comment}

\textbf{
\begin{itemize}
\item The system has to be lightweight and resource efficient.
\item Protect the host OS and its trusted applications from an untrusted app while
it is executing in an isolated, sanitized environment.
\item Have the ability to support unmodified apps (paid or otherwise).
\item At any point in time, various groups of apps could be executing in different isolated
environments but a unified user experience still exists.
\end{itemize}
}


==> evaluation.tex <==
\section{Performance Evaluation}
\label{sec:experiments}



\subsection{Headless Architecture}
The use of a headless architecture has tradeoffs. UI events get
handled more efficiently but system calls that are transferred to
the guest virtual machine require more overheads. In an alternative
design where the entire application is encapsulated, UI events become
more expensive as they have to be sent over a remote window protocol, e.g.,
see Drawbridge~\cite{drawbridge}.

To validate ur hypothesis that handling UI efficiently is a better
strategy, we measured the frequency of display and touch events as compared
to other class of events for several popular applications.
We ran 5 regular applications available - Email, Web Browser, Music, MMS, Default Game.  
As we see in Table \ref{tab:ioctlstats}, over 92\% of the system calls made are
UI-related.  A similar study measuring categories of system calls was
conducted by ProfileDroid \cite{Wei:2012:PMP:2348543.2348563} as
well. The results from both studies serve to confirm our hypothesis.

\begin{table}[ht!] \center
\begin{tabular}{| l | c | c |}
\hline
Service Requested			& Total Count	& Percent	\\ \hline
\hline
android.accounts			& 2		& 0.00\%	\\ \hline
android.app				& 1769		& 2.96\%	\\ \hline
android.content				& 1611		& 2.69\%	\\ \hline
android.media				& 16		& 0.03\%	\\ \hline
android.net				& 4		& 0.01\%	\\ \hline
android.os				& 122		& 0.20\%	\\ \hline
android.ui				& 48646		& 81.35\%	\\ \hline
android.utils				& 919		& 1.54\%	\\ \hline
android.view				& 2004		& 3.35\%	\\ \hline
com.android.internal.telephony		& 82		& 0.14\%	\\ \hline
com.android.internal.view		& 4619		& 7.72\%	\\ \hline
ImountService				& 1		& 0.00\%	\\ \hline
\end{tabular}
\caption{Counts of various Binder IPC ioctls issued to Android services.
Note that UI dominates other types of requests.}
\label{tab:ioctlstats}
\end{table}

Next, we run a microbenchmark to analyze the overhead of the
VM-independent system call interception framework.  We run two popular
Android macrobenchmarks to analyze whole system performance and one
application level benchmark to analyze the impact on end users. The
macrobenchmarks are used so that we can measure the performance for
interactive workloads that are the most common for smartphones. We
also report on the memory consumption of the guest VMs.

All the benchmarks are run on an Asus EEEPC ET1602 equipped with an
Intel Atom x86 processor, 1GB of RAM and 160GB of internal flash
memory. The EEEPC runs Android x86 version 2.3.7 with Linux kernel
version 2.6.39.  We configured the guest VM with 64MB of main memory
that ran our headless Android port.

\subsection{Microbenchmarks2}
\label{perf}
%microbench for syscall intercept, ping-pong
%app bench
%graphics macro bench details, with opaque overall nums
%fs microbench r/w
We run a microbenchmark to measure the latency of performing 3 common system calls with the Anception Syscall Interception Method (ASIM) activated.
We measure the time for a \textit{null-redirection}, which is intercepting a syscall and
redirecting it to the real system call handler.
The benchmark executes the syscalls 10,000 times and uses the x86 cycle counter for timing.
Trial runs are executed by the benchmark to warm up the caches. The results for the ASIM are summarized
in Table \ref{asim}. The write, read calls are executed on files.

\begin{table}[ht!]
\center
\begin{tabular}{| l | c | c |}

   	\hline
   	syscall							&							Native ($\mu s$)						& 					Anception ($\mu s$) \\ \hline
   	getpid							&						0.57									& 					0.57 \\ \hline
   	write (32 bytes)		&						17.7								&						17.8 \\ \hline
   	read (32 bytes)			&						3.3									&						3.4 \\ \hline
\end{tabular}
\caption{ASIM latency}
\label{asim}
\end{table}

%\vspace{-0.2in}

As we can see in the table, the ASIM adds negligible overhead and is very efficient.
The next microbenchmark measures the round-trip time for a system call when redirected to an active guest VM.
The results are summarized in Table \ref{rtt}.

\begin{table}[ht!]
\center
\begin{tabular}{| l | c | c |}

   	\hline
   	syscall							&							Native ($\mu s$)						& 					Anception ($\mu s$) \\ \hline
   	write (16 bytes)		&						24.9								&						206.9 \\ \hline
   	read (16 bytes)			&						3.4								&						203.2 \\ \hline
   	write (32 bytes)		&						17.7									&						196.6 \\ \hline
   	read (32 bytes)			&						3.3									&						212.7 \\ \hline
   	
\end{tabular}
\caption{Full redirection round trip time}
\label{rtt}
\end{table}

%\vspace{-0.2in}

The increase in latency is caused due to two VM switches (host -> guest, guest -> host) and process context switches.
As context switch times go down due to improvements in hypervisor technology, we expect to see reductions in the latency. However, these numbers do not adversely affect performance
at a macro level, which is what we report on next.

\subsection{Macrobenchmarks}
We run three popular Android macrobenchmarks -- PassMark \cite{passmark}, AnTuTu \cite{antutu} and SunSpider \cite{sunspider}. These benchmarks are designed to test 2D and 3D graphics
performance, Disk I/O, Memory I/O and CPU (Java, Native) performance. They report a weighted total score, and individual scores.
Running 2D/3D benchmarks enables us to analyze the overheads caused by our \texttt{ioctl} handling logic. It should not cause
a large overhead because graphics related \texttt{ioctls} form a large chunk of the system 
calls executed by applications (Table \ref{tab:ioctlstats}).

%Also, Android allows users to play many games and under Anception, we should not have large overheads for
%such activities.

\begin{comment}
In Table \ref{antutu}, we report the total score alongwith the graphics and memory I/O scores.

\begin{table}[ht!]
\center
\begin{tabular}{| l | c | c |}
		\hline
		AnTuTu Test							&							Native						& 					Anception \\ \hline
	  Total 								&			5408											& 5214								\\ \hline		
	  Memory I/O 					&			1190											& 1190					   		\\ \hline
	  2D Graphics 					&     251												& 250								\\ \hline
	  3D Graphics 					&     539												& 532                 \\ \hline
	  
\end{tabular}
\caption{AnTuTu Macro Benchmark}
\label{antutu}
\end{table}
\end{comment}

\begin{comment}
%
	  %Total 								&			5430											& 5226								\\ \hline		
	  %Memory I/O 					&			1191											& 1190					   		\\ \hline
	  %2D Graphics 					&     251												& 253									\\ \hline
	  %3D Graphics 					&     554												& 530                 \\ \hline
	  %\hline
\end{comment}

The PassMark benchmark reports details of the tests conducted. Figure \ref{passmark}
shows us that Anception incurs negligible overhead for a range of 2D and 3D graphics tests.
They also show no noticeable change. Overhead of 3.88\% is incurred on 2D tests and 2.64\% on 3D tests. In terms of CPU and Memory I/O, as reported by PassMark,
Anception incurs 0.43\% overhead on memory operations and 2.3\% overhead on CPU operations.
This slight increase is due to the guest VM running Headless Android that puts additional scheduling and 
memory pressure on the host. However, due to our architecture of handling UI operations on the host,
the impact of this VM is negligible. 

\begin{figure}[ht!]
\center
\includegraphics[width=3.6in,height=3.5in,keepaspectratio]{graphs/passmark.pdf}
\caption{PassMark Benchmark}
\label{passmark}
\end{figure}

On the AnTuTu Benchmark, Anception's score was 3.6\% less than native, with a 0.4\% overhead on the 2D tests and 1.3\% overhead on the 3D tests.
To get an idea of Anception's performance with interactive and application oriented workloads,
we run the SunSpider \cite{sunspider} Benchmark. At a macro level, from Figure \ref{sunspider}, we observe
that Anception closely follows the performance of native execution with a 1.2\% maximum overhead among all tests. This benchmark also shows our ability to run unmodified
Android applications on Anception. The reason for the modest overheads is the \texttt{ioctl} identification code wherein we
determine whether a particular IPC operation is related to graphics and input operations.

\begin{figure}[ht!]
\center
\includegraphics[width=3.6in,height=3.5in,keepaspectratio]{graphs/sunspider.pdf}
\caption{SunSpider Benchmark -- Time in milliseconds}
\label{sunspider}
\end{figure}

\subsection{Memory overhead}
Finally, we quantify the memory (RAM) savings earned by using a headless version of Android. To measure this,
we read the \texttt{/proc/meminfo} file on a stock Android 2.3.7 system, and we read the meminfo file
on a headless instance. These readings were taken when the systems were just booted up and just the bare essentials
were running.
For a stock Android system, the number of active bytes of memory is 99.11 MB.
On the headless version, it is 14.87 MB, or 15\% of stock Android. This is much smaller compared
to 40\% of stock Android that is needed by Cells to start a guest VM. Moreover, we have not applied
optimizations like Kernel Samepage Merging (KSM) that Cells has applied to its implementation. We expect
to see further reductions with KSM in place.
The reason for the decrease is again due to Anception's architecture.
By running a Headless Android instance in the guest VM, the memory used up by Display Managers and Input Managers
is freed up, allowing us to run smaller sized (in terms of RAM) VMs. However, during all our experiments, we started
the guest VMs with 64MB of main memory, although we could have started them with as low as 44MB of memory. We did not
do this as we didn't want to adjust the Android low memory killer parameters.

\subsection{Power Measurements}
\hl{Antutu is cited below but its data is missing}
Smart phones are resource constrained devices and usually suffer with limited battery power. In order to ensure that the
effect on energy consumption due to Anception is not significant, we conducted experiments on PassMark and AnTuTu benchmars to quantify 
the overheads. We used a Watts Up? .Net power meter for our measurements on power and energy consumption. Using the MonkeyRunner 
feature provided by the Android platform, we built automated tests to run the benchmarks for approximately an hour each, both with 
and without Anception enabled. In order to simulate the actual execution of an application, the benchmark was exited using the back button 
after every run. For the PassMark benchmark, we observed that the energy consumption was 20.8 Watt hours without binding it to Anception 
and the consumption went upto 21.3 Watt hours upon binding, giving an overhead of 2.4\%. 


